Surround-View Cameras based Holistic Visual Perception for Automated Driving

The formation of eyes led to the big bang of evolution. The dynamics changed from a primitive organism waiting for the food to come into contact for eating food being sought after by visual sensors. The human eye is one of the most sophisticated developments of evolution, but it still has defects. Humans have evolved a biological perception algorithm capable of driving cars, operating machinery, piloting aircraft, and navigating ships over millions of years. Automating these capabilities for computers is critical for various applications, including self-driving cars, augmented reality, and architectural surveying. Near-field visual perception in the context of self-driving cars can perceive the environment in a range of $0-10$ meters and 360{\deg} coverage around the vehicle. It is a critical decision-making component in the development of safer automated driving. Recent advances in computer vision and deep learning, in conjunction with high-quality sensors such as cameras and LiDARs, have fueled mature visual perception solutions. Until now, far-field perception has been the primary focus. Another significant issue is the limited processing power available for developing real-time applications. Because of this bottleneck, there is frequently a trade-off between performance and run-time efficiency. We concentrate on the following issues in order to address them: 1) Developing near-field perception algorithms with high performance and low computational complexity for various visual perception tasks such as geometric and semantic tasks using convolutional neural networks. 2) Using Multi-Task Learning to overcome computational bottlenecks by sharing initial convolutional layers between tasks and developing optimization strategies that balance tasks.

==> Figures/omnidet/motion/motion.tex <==
\begin{comment}
\newcommand{\turnheightnew}{0.4\columnwidth}
\centering
\begin{adjustbox}{max width=0.78\textwidth}
\begin{tabular}{@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}}

{\rotatebox{90}{\hspace{13mm} \Large Front Cam (t-6)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180524.110553_FV_271_t_6.jpg} &
{\rotatebox{90}{\hspace{13mm} \Large Rear Cam (t-6)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180524.143632_RV_361_t_6.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Front Cam (t)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180524.110553_FV_271_t.jpg} &
{\rotatebox{90}{\hspace{13mm} \Large Rear Cam (t)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180524.143632_RV_361_t.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Motion Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180524.110553_FV_271_motion.jpg} &
{\rotatebox{90}{\hspace{13mm} \Large Motion Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180524.143632_RV_361_motion.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Left Cam (t-6)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180821.113442_MVL_481_t_6.jpg} &
{\rotatebox{90}{\hspace{13mm} \Large Right Cam (t-6)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180529.123717_MVR_361_t_6.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Left Cam (t)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180821.113442_MVL_481_t.jpg} &
{\rotatebox{90}{\hspace{13mm} \Large Right Cam (t)}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180529.123717_MVR_361_t.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Motion Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180821.113442_MVL_481_motion.jpg} &
{\rotatebox{90}{\hspace{13mm} \Large Motion Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/motion/W213-263.YUV.4CAM.DAT.20180529.123717_MVR_361_motion.jpg} \\

\end{tabular}
\end{adjustbox}
\end{comment}

==> Figures/omnidet/norm_cyl/norm_cyl.tex <==
\newcommand{\turnheightnew}{0.42\columnwidth}
\centering
\begin{adjustbox}{max width=0.78\textwidth}
\begin{tabular}{@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{\hskip 0.4mm}c@{}}

{\rotatebox{90}{\hspace{13mm} \Large Front Camera}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180526.131954_FV_271_.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180601.114840_FV_301_.jpg} \\

{\rotatebox{90}{\hspace{9mm} \Large Distance Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180526.131954_FV_271_norm_motion.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180601.114840_FV_301_norm_motion.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Left Camera}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180524.140432_MVL_331_.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180527.112658_MVL_61_.jpg} \\

{\rotatebox{90}{\hspace{9mm} \Large Distance Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180524.140432_MVL_331_norm_motion.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180527.112658_MVL_61_norm_motion.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Right Camera}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180531.145708_MVR_871_.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180601.163419_MVR_361_.jpg} \\

{\rotatebox{90}{\hspace{9mm} \Large Distance Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180531.145708_MVR_871_norm_motion.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180601.163419_MVR_361_norm_motion.jpg} \\

{\rotatebox{90}{\hspace{13mm} \Large Rear Camera}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180524.125332_RV_211_.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180531.160224_RV_1711_.jpg} \\

{\rotatebox{90}{\hspace{9mm} \Large Distance Estimate}} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180524.125332_RV_211_norm_motion.jpg} &
\includegraphics[height=\turnheightnew]{Figures/omnidet/norm_cyl/W213-263.YUV.4CAM.DAT.20180531.160224_RV_1711_norm_motion.jpg} \\

\end{tabular}
\end{adjustbox}

==> Figures/svdistnet/post_processing/nform/post_processing_v1.tex <==
\centering
\begin{tabular}{@{\hskip 0.5mm}c@{}}

\includegraphics[height=\textwidth]{Figures/svdistnet/post_processing/vlcsnap-2020-09-07-11h50m49s962.png} \\
\includegraphics[height=\textwidth]{Figures/svdistnet/post_processing/vlcsnap-2020-09-07-11h51m31s816.png} \\
\includegraphics[height=\textwidth]{Figures/svdistnet/post_processing/vlcsnap-2020-09-07-11h52m13s070.png} \\

\end{tabular}


==> Figures/svdistnet/post_processing/nform/post_processing_v2.tex <==
\centering
\begin{tabular}{@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{\hskip 0.5mm}c@{}}

\includegraphics[height=\textwidth]{Figures/svdistnet/post_processing/vlcsnap-2020-09-07-11h53m42s103_crop.jpg} \\
\includegraphics[height=\textwidth]{Figures/svdistnet/post_processing/vlcsnap-2020-09-07-11h52m41s488_crop.jpg} \\
\includegraphics[height=\textwidth]{Figures/svdistnet/post_processing/vlcsnap-2020-09-07-11h53m58s395_crop.jpg} \\
\end{tabular}


==> Results/omnidet/cgt_effect.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Ablation study on the effect of CGT contributions} up to our final OmniDet model on Woodscape.}
\label{table:cgt_effect}
\scalebox{0.8}{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{ccccccccc}
\toprule
  \textit{\begin{tabular}[c]{@{}c@{}}Semantic\\ Guide Dist.\end{tabular}} &
  \textit{\begin{tabular}[c]{@{}c@{}}Semantic\\ Mask\end{tabular}} &
  \textit{\begin{tabular}[c]{@{}c@{}}Motion\\ Mask\end{tabular}} &
  \textit{\begin{tabular}[c]{@{}c@{}}Semantic\\ Guide Det.\end{tabular}} &
  \textit{CGT} &
  \cellcolor[HTML]{00b0f0}\textbf{\textit{RMSE} $\mathbf{\downarrow}$} &
  \multicolumn{1}{c}{\cellcolor[HTML]{00b050}\begin{tabular}[c]{@{}c@{}}\textbf{\textit{mIoU}}\\ \textbf{\textit{Seg}} \end{tabular}} &
  \multicolumn{1}{c}{\cellcolor[HTML]{ab9ac0}\begin{tabular}[c]{@{}c@{}}\textbf{\textit{mIoU}}\\ \textbf{\textit{Mot.}}\end{tabular}} &
  \multicolumn{1}{c}{\cellcolor[HTML]{a5a5a5}\begin{tabular}[c]{@{}c@{}}\textbf{\textit{mAP}}\\ \textbf{\textit{Det}}\end{tabular}} \\
\midrule
\xm & \xm & \xm & \xm & \xm & 1.764 & 73.6 & 72.3 & 63.5 \\  
\xm & \xm & \xm & \xm & \ch & \textbf{1.681} & \textbf{74.2} & \textbf{73.5} & \textbf{63.8} \\  
\ch & \ch & \xm & \xm & \xm & 1.512 & 74.5 & 73.4 & 63.6 \\  
\ch & \ch & \xm & \xm & \ch & \textbf{1.442} & \textbf{74.8} & \textbf{74.0} & \textbf{64.1} \\   
\ch & \xm & \ch & \xm & \xm & 1.397 & 75.2 & 74.3 & 64.0 \\
\ch & \xm & \ch & \xm & \ch & \textbf{1.352} & \textbf{75.5} & \textbf{74.8} & \textbf{64.3} \\ 
\ch & \xm & \ch & \ch & \xm & 1.348 & 75.9 & 74.9 & 67.8 \\   
\ch & \xm & \ch & \ch & \ch & \textbf{1.332} & \textbf{76.6} & \textbf{75.3} & \textbf{68.4} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> Results/svdistnet/optimizer.tex <==
\begin{table}[!ht]
\centering
\small
\begin{adjustbox}{width=0.75\columnwidth}
\setlength{\tabcolsep}{0.2em}
  \begin{tabular}{lccccccc}
	\toprule
    \multirow{2}{*}{\textbf{Optimizer}} &
    \cellcolor[HTML]{7d9ebf}Abs Rel & \cellcolor[HTML]{7d9ebf}Sq Rel & \cellcolor[HTML]{7d9ebf}RMSE & \cellcolor[HTML]{7d9ebf}RMSE$_{log}$ & \cellcolor[HTML]{e8715b}$\delta<1.25$ & \cellcolor[HTML]{e8715b}$\delta<1.25^2$ & \cellcolor[HTML]{e8715b}$\delta<1.25^3$ \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-8}
    &  \multicolumn{4}{c}{\cellcolor[HTML]{7d9ebf}lower is better} & \multicolumn{3}{c}{\cellcolor[HTML]{e8715b}higher is better} \\
    \toprule
     Adam    & 0.069 & 0.338 & 1.551 & 0.118 & 0.887 & 0.980 & 0.991 \\
     Ranger  & 0.057 & 0.315 & 1.532 & 0.108 & 0.896 & 0.987 & 0.996 \\
    \bottomrule
  \end{tabular}
\end{adjustbox}
\caption{\textbf{Impact of the optimizer} on WoodScape dataset.~\cite{yogamani2019woodscape}.}
\label{table:optimizer}
\end{table}

==> Results/svdistnet/robust_loss_ablation.tex <==
\begin{table}[t!]
\captionsetup{belowskip=0pt, skip=4pt, font= small, singlelinecheck=false}
\centering
  \small
  \begin{adjustbox}{width=0.75\columnwidth}
    \setlength{\tabcolsep}{0.1em}
	  \begin{tabular}{llccccccc}
	    \toprule
        \multirow{2}{*}{\textbf{Method}}  & \multirow{2}{*}{$\rho$} & \cellcolor[HTML]{7d9ebf}Abs Rel & \cellcolor[HTML]{7d9ebf}Sq Rel & \cellcolor[HTML]{7d9ebf}RMSE & \cellcolor[HTML]{7d9ebf}RMSE$_{log}$ & \cellcolor[HTML]{e8715b}$\delta<1.25$ & \cellcolor[HTML]{e8715b}$\delta<1.25^2$ & \cellcolor[HTML]{e8715b}$\delta<1.25^3$ \\
        \cmidrule(lr){3-6} \cmidrule(lr){7-9}
        & & \multicolumn{4}{c}{\cellcolor[HTML]{7d9ebf}lower is better} & \multicolumn{3}{c}{\cellcolor[HTML]{e8715b}higher is better} \\
	    \toprule
	    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SynDistNet \end{tabular}}   
	    & 2    & 0.154 & 0.631 & 2.532 & 0.198 & 0.832 & 0.965 & 0.981 \\
        & 0, 2 & 0.142 & 0.537 & 2.316 & 0.179 & 0.878 & 0.971 & 0.985 \\
        \midrule
        \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}} SVDistNet \end{tabular}}       
        & 2    & 0.145 & 0.564 & 2.279 & 0.186 & 0.863 & 0.966 & 0.982 \\
        & 0, 2 & 0.128 & 0.469 & 2.153 & 0.164 & 0.875 & 0.974 & 0.986 \\
	   \bottomrule
    \end{tabular}
  \end{adjustbox}
\caption[\bf Impact of using the robust loss function in SynDistNet and SVDistNet.]
{\textbf{Impact of using the robust loss function} compared to the baseline from \cite{kumar2020syndistnet} on the WoodScape dataset.}
\label{table:svdistnet-robust-ablation}
\end{table}


==> Results/syndistnet/features_ablation.tex <==
\begin{table*}[!ht]
  \centering{
  \small
  \begin{adjustbox}{width=\columnwidth}
  \setlength{\tabcolsep}{0.3em}
  \begin{tabular}{l|c|c|c|c|cccc|ccc}
    \toprule
      \multirow{2}{*}{
       \textbf{Network} } & 
       \multirow{2}{*}{\emph{RL}} &
       \multirow{2}{*}{\emph{Self-Attn}} & 
       \multirow{2}{*}{\emph{SEM}} & 
       \multirow{2}{*}{\emph{Mask}} & 
       \multicolumn{4}{c|}{\cellcolor[HTML]{7d9ebf}Lower is Better} & 
       \multicolumn{3}{c}{\cellcolor[HTML]{e8715b}Higher is Better} \\
        & & &  &     & \cellcolor[HTML]{7d9ebf}Abs Rel & \cellcolor[HTML]{7d9ebf}Sq Rel & \cellcolor[HTML]{7d9ebf}RMSE & \cellcolor[HTML]{7d9ebf}RMSE$_{log}$ & \cellcolor[HTML]{e8715b}$\delta < 1.25$ & \cellcolor[HTML]{e8715b}$\delta < 1.25^2$ & \cellcolor[HTML]{e8715b}$\delta < 1.25^3$ \\
       \toprule
       FisheyeDistanceNet \cite{kumar2020fisheyedistancenet} & \xm & \xm & \xm & \xm & 0.152 & 0.768 & 2.723 & 0.210 & 0.812 & 0.954 & 0.974 \\
       \midrule
        \multirow{6}{*}{SynDistNet (ResNet-18)}
        & \ch & \xm & \xm & \xm & 0.142 & 0.537 & 2.316 & 0.179 & 0.878 & 0.971 & 0.985 \\
        & \ch & \xm & \xm & \ch & 0.133 & 0.491 & 2.264 & 0.168 & 0.868 & 0.976 & 0.988 \\
        & \ch & \ch & \xm & \ch & 0.121 & 0.429 & 2.128 & 0.155 & 0.875 & 0.980 & 0.990 \\
        & \ch & \ch & \ch & \xm & 0.105 & 0.396 & 1.976 & 0.143 & 0.878 & 0.982 & 0.992 \\
        & \ch & \ch & \ch & \ch & \textbf{0.076} & \textbf{0.368} & \textbf{1.714} & \textbf{0.127} & \textbf{0.891} & \textbf{0.988} & \textbf{0.994} \\
        \midrule
        \multirow{6}{*}{SynDistNet (ResNet-50)}
        & \ch & \xm & \xm & \xm & 0.138 & 0.540 & 2.279 & 0.177 & 0.880 & 0.973 & 0.986 \\
        & \ch & \xm & \xm & \ch & 0.127 & 0.485 & 2.204 & 0.166 & 0.881 & 0.975 & 0.989 \\
        & \ch & \ch & \xm & \ch & 0.115 & 0.413 & 2.028 & 0.148 & 0.876 & 0.983 & 0.992 \\
        & \ch & \ch & \ch & \xm & 0.102 & 0.387 & 1.856 & 0.135 & 0.884 & 0.985 & 0.994 \\
        & \ch & \ch & \ch & \ch & \textbf{0.068} & \textbf{0.352} & \textbf{1.668} & \textbf{0.121} & \textbf{0.895} & \textbf{0.990} & \textbf{0.996} \\
   \bottomrule
  \end{tabular}
  \end{adjustbox}
  }
\caption[\bf Ablative analysis showing the effect of each of our contributions using the WoodScape dataset in SynDistNet framework.]
 {\textbf{Ablative analysis} showing the effect of each of our contributions using the WoodScape dataset. The input resolution is $512 \times 256$ pixels and distances are capped at $40\,m$. We start with FisheyeDistanceNet \cite{kumar2020fisheyedistancenet} baseline and incrementally add robust loss (RL), self-attention based encoder (Self-Attn), semantically-guided decoder (SEM) and dynamic object masking (Mask).}
\label{table:syndistnet-table_ablation}
\end{table*}

==> Results/syndistnet/mtl.tex <==
\begin{table}[!ht]
  \centering
    \begin{adjustbox}{width=0.7\columnwidth}
      \begin{tabular}{l|c|c}
      \toprule
      \multicolumn{1}{l|}{\textbf{Model}} 
      & \multicolumn{1}{c|}{\cellcolor[HTML]{00b050}\begin{tabular}[c]{@{}c@{}}\textit{Segmentation} \\ (mIOU)\end{tabular}} & \multicolumn{1}{c}{\cellcolor[HTML]{00b0f0}\begin{tabular}[c]{@{}c@{}} \textit{Distance} \\ (RMSE) \end{tabular}} \\ 
      \midrule 
      Segmentation only baseline     & 76.8         & \xm   \\ 
      Distance only baseline         & \xm          & 2.316 \\ 
      MTL baseline                   & 78.3         & 2.128 \\ 
      MTL with synergy (SynDistNet) & \textbf{81.5} & \textbf{1.714} \\ 
      \bottomrule
    \end{tabular}
\end{adjustbox}
\caption{\textbf{Multi-task learning (MTL) ablation results} on the WoodScape dataset using a ResNet18 encoder.}
\label{tab:syndistnet-mtl}
\end{table}
